Quantifying First-Order Markov Violations in Noisy Reinforcement Learning: A Causal Discovery Approach

Reinforcement learning (RL) methods frequently assume that each new observation completely reflects the environment's state, thereby guaranteeing Markovian (one-step) transitions. In practice, partial observability or sensor/actuator noise often invalidates this assumption. This paper proposes a systematic methodology for detecting such violations, combining a partial correlation-based causal discovery process (PCMCI) with a novel Markov Violation score (MVS). The MVS measures multi-step dependencies that emerge when noise or incomplete state information disrupts the Markov property. Classic control tasks (CartPole, Pendulum, Acrobot) serve as examples to illustrate how targeted noise and dimension omissions affect both RL performance and measured Markov consistency. Surprisingly, even substantial observation noise sometimes fails to induce strong multi-lag dependencies in certain domains (e.g., Acrobot). In contrast, dimension-dropping investigations show that excluding some state variables (e.g., angular velocities in CartPole and Pendulum) significantly reduces returns and increases MVS, while removing other dimensions has minimal impact. These findings emphasize the importance of locating and safeguarding the most causally essential dimensions in order to preserve effective single-step learning. By integrating partial correlation tests with RL performance outcomes, the proposed approach precisely identifies when and where the Markov assumption is violated. This framework offers a principled mechanism for developing robust policies, informing representation learning, and addressing partial observability in real-world RL scenarios. All code and experimental logs are accessible for reproducibility (https://github.com/ucsb/markovianess).

==> backups/related_works.tex <==
\section{Related Works}
\label{sec:related-works}

Real‐world reinforcement learning (RL) often encounters partial observability and noisy signals that deviate from the ideal Markov property \cite{wiering_partially_2012}. This section surveys \emph{robust RL} and \emph{learning from noisy data}, then highlights \emph{causal discovery} approaches for detecting non‐Markovian effects. In contrast to earlier studies limited to specific noise models or post‐hoc performance metrics, the present work introduces a unified \emph{Markov Violation Score} (MVS) that quantifies multi‐step dependencies arising under observation and action perturbations.

\subsection{Robust RL and Learning from Noisy Data}
Past research has developed robust RL algorithms capable of withstanding disturbances in transitions or observations~\cite{panaganti_robust_2022, liu_distributionally_2022}, along with methods such as \emph{adversarial training}\cite{pinto_robust_2017} or \emph{domain randomization} for visual noise or reward shaping~\cite{wang_robust_2019, li_mural_2021, wang_reinforcement_2020}. Other works investigate noisy rewards~\cite{wang_reinforcement_2020} or add noise to observations/actions~\cite{hollenstein_colored_2024, hollenstein_action_2023, igl_generalization_2019}, often assuming a known noise model. By contrast, the methodology here applies PCMCI~\cite{runge_discovering_2022} in a model‐free manner, detecting lag‐2+ dependencies within trajectory data to reveal when first‐order Markov assumptions break.

\subsection{Causal Discovery and Testing the Markov Assumption}
Constraint‐based \emph{causal discovery} methods (e.g., the PC algorithm~\cite{spirtes_causation_2001}) use conditional‐independence tests to prune graphs. A \emph{momentary conditional independence (MCI)} variant extends these ideas to time‐lagged RL data~\cite{zhu_causal_2020}, forming the foundation of PCMCI. Previous studies have examined whether the Markov property holds~\cite{shi_does_2020}, though usually without a metric quantifying how severely it is violated. In this work, \textbf{PCMCI} identifies multi‐lag links in RL rollouts, while the \emph{Markov Violation Score (MVS)} aggregates those links into a single measure reflecting deviation strength.

\subsection*{How This Work Differs}
\begin{itemize}
    \item \emph{Quantifying Markov Violations:} Rather than focusing only on final returns, the Markov Violation Score (MVS) captures higher‐order dependencies to clarify \emph{why} performance degrades.
    \item \emph{Dimension‐Specific Vulnerabilities:} Noise or omissions targeting specific dimensions demonstrate which state or action components uphold first‐order Markov structure.
    \item \emph{Linking Causal Structure and RL:} Surges in lag‐2+ partial correlations often coincide with policy collapse, indicating a breakdown in single‐step assumptions.
    \item \emph{Action‐Space Insights:} Discrete‐action tasks (CartPole, Acrobot) sometimes exhibit more dramatic Markov failures than continuous‐action tasks (Pendulum).
\end{itemize}

Overall, while robust RL~\cite{panaganti_sample_2022}, noise tolerance~\cite{wang_reinforcement_2020}, and causal discovery~\cite{spirtes_causation_2001} have been extensively explored, this work integrates them by leveraging PCMCI and a Markov Violation Score to pinpoint multi‐lag dependencies and safeguard crucial dimensions for sustaining high performance. 

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

%--------------------------------------------------------------------
\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    The abstract and \S\ref{sec:introduction} concisely state the two core contributions—(i) the Markov-Violation Score (MVS) and (ii) an empirical study on three classic control tasks under various noise/omission scenarios—and do not claim results beyond this scope.

%--------------------------------------------------------------------
\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    \S\ref{sec:limitations-future} details task breadth, algorithm coverage (PPO only), linear-test assumptions, and real-world realism as explicit limitations.

%--------------------------------------------------------------------
\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification:  
    The paper is empirical and introduces no formal theorems.

%--------------------------------------------------------------------
\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    \S\ref{sec:setup} lists all PPO hyper-parameters, training budgets and environments; \S\ref{sec:seeds-ci} gives the seed protocol; a full JSON config and scripts are linked in the public repository.

%--------------------------------------------------------------------
\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    A GitHub link (to be anonymised for review) contains all source code, configs, and plotting scripts; all tasks use the open-source Gymnasium benchmark environments.

%--------------------------------------------------------------------
\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    Hyper-parameters (\S\ref{sec:setup}), seed choice and CI computation (\S\ref{sec:seeds-ci}), and PCMCI settings (config JSON in repo) are fully enumerated.

%--------------------------------------------------------------------
\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars or other significance information?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    \S\ref{sec:seeds-ci} explains that each condition is run with five seeds and reports mean $\pm$95\%~CI; tables in are reported in source code as csv.

%--------------------------------------------------------------------
\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    All runs were executed on a single Apple M3 Pro laptop (12-core CPU, 18 GB RAM, macOS 14) with no discrete GPU.  
    A 50 k-step CartPole/Acrobot job completes in 3 min wall-clock; the 450 k-step Pendulum job takes 40 min.  
    The full study (three tasks, all variants, five seeds each) required 25 CPU-hours.

%--------------------------------------------------------------------
\item {\bf Code of ethics}
    \item[] Question: Does the research conform with the NeurIPS Code of Ethics?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    The work uses only publicly available simulators and releases code under an open-source license; no privacy-sensitive or human data are involved.

%--------------------------------------------------------------------
\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both positive and negative societal impacts?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    \S\ref{sec:limitations-future} highlights MVS as a potential safety diagnostic for real robots (positive) and warns of over-confidence if mis-interpreted (negative).

%--------------------------------------------------------------------
\item {\bf Safeguards}
    \item[] Question: Are safeguards described for high-risk data/models?
    \item[] Answer: \answerNA{}
    \item[] Justification:  
    No high-risk data or large generative models are released.

%--------------------------------------------------------------------
\item {\bf Licenses for existing assets}
    \item[] Question: Are existing assets properly credited and licensed?
    \item[] Answer: \answerYes{}
    \item[] Justification:  
    Gymnasium, Stable-Baselines3, and PCMCI-Py are cited with their MIT or BSD licenses.

%--------------------------------------------------------------------
\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented?
    \item[] Answer: \answerNA{}
    \item[] Justification:  
    The study releases only code; no new datasets or models are introduced.

%--------------------------------------------------------------------
\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: Does the paper include full instructions and screenshots?
    \item[] Answer: \answerNA{}
    \item[] Justification:  
    No human-subject or crowdsourcing data were collected.

%--------------------------------------------------------------------
\item {\bf Institutional review board (IRB) approvals}
    \item[] Question: Does the paper describe participant risks and IRB approval?
    \item[] Answer: \answerNA{}
    \item[] Justification:  
    Not applicable—no human subjects.

%--------------------------------------------------------------------
\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe usage of LLMs if relevant?
    \item[] Answer: \answerNA{}
    \item[] Justification:  
    Large language models are not part of the methodology.

\end{enumerate}
